MechaTerp-TRACE: A Novel Approach for Component Ablation Analysis in Language Models

Interpretability research on large language models has produced accounts of factual recall in feed-forward layers and of token relationships in self-attention, but little work offers a unified way to compare the causal contribution of different architecture components to a model's output. We introduce MechaTerp (the Mechanistic Interpretability suite) -TRACE (subset for Teacher-forced Registry of Ablated Component Effects), an architecture and study that measures how much each registered component of a language model supports the production of a named entity. TRACE ablates one component at a time and measures the resulting change in the output distribution at a fixed answer token, so component types from whole transformer blocks down to individual neurons and output logits can be compared on a common scale. We apply it to thirteen instruction-tuned dense decoder models spanning five families and one to thirty billion parameters, ablating 49,656 components across 48 medical and 42 general-knowledge prompts. We find that the components carrying the most effect are the same few, positionally fixed components in every model, regardless of which entity a prompt asks about, and that once these are removed, the remaining support is close to evenly spread in eleven of the thirteen models. Apparent localisation of entity knowledge is therefore largely attributable to generic generation machinery, which has direct consequences for methods that assume entity knowledge sits in a findable place, including targeted knowledge editing.

==> subpages/results_combined_no_gemma_old.tex <==
% Requires in the document preamble: \usepackage{booktabs,multirow,threeparttable,caption}
% Designed to \input{} as-is inside a two-column document (table* spans both columns).
% Plain 'r' (right-aligned) columns throughout, not siunitx S: with models as
% columns, each column mixes params/counts/LLI/p-values, so numbers are
% pre-formatted to fixed precision in the generator rather than relying on a
% single numeric column type. Upright table*, not rotated -- 13 model columns
% (after dropping Gemma) fit without landscaping; see the width estimate printed
% by the generator script.
\begin{table*}[t]
\centering
\captionsetup{font=small}
\caption{MechaTerp-TRACE per-model results (13 models; Gemma excluded from this cohort), combining localisation (Eq. 5), cross-prompt reuse (Eq. 6), and domain-common/generation-floor components with their LLI correction (Eq. 9, 11, 12), transposed with models as columns. Short labels (family-Params): Gr-3B=Granite-4.1-3B, Gr-8B=Granite-4.1-8B, Gr-30B=Granite-4.1-30B, L-1B=Llama-3.2-1B, L-3B=Llama-3.2-3B, L-8B=Llama-3.1-8B-Instruct, Mi-7B=Mistral-7B-Instruct-v0.2, Mn-3B=Ministral-3B, MP=MediPhi-Clinical, Ph=Phi-4-mini, Q-1.7B=Qwen3-1.7B, Q3.5-9B=Qwen3.5-9B, Q3.5-2B=Qwen3.5-2B. }
\label{tab:results-combined-no-gemma}
\footnotesize
\setlength{\tabcolsep}{2.5pt}
\begin{threeparttable}
\begin{tabular}{lrrrrrrrrrrrrr}
\toprule
{} & \multicolumn{3}{c}{Granite} & \multicolumn{3}{c}{Llama} & \multicolumn{2}{c}{Mistral} & \multicolumn{2}{c}{Phi} & \multicolumn{3}{c}{Qwen} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-14}
{Metric} & Gr-3B & Gr-8B & Gr-30B & L-1B & L-3B & L-8B & Mi-7B & Mn-3B$^\dagger$ & MP & Ph & Q-1.7B & Q3.5-9B & Q3.5-2B \\
\midrule
\multicolumn{14}{l}{\textbf{Identity}} \\
\midrule
Params & 3B & 8B & 30B & 1B & 3B & 8B & 7B & 3B & 3.8B & 3.8B & 1.7B & 9B & 2B \\
$B$ (block-lane size) & 40 & 40 & 64 & 16 & 28 & 32 & 32 & 14 & 32 & 32 & 28 & 32 & 24 \\
\midrule
\multicolumn{14}{l}{\textbf{Correctness}} \\
\midrule
Correct (of 90) & 63 & 75 & 77 & 46 & 71 & 68 & 72 & 0 & 71 & 64 & 35 & 57 & 55 \\
Med. correct (of 48) & 29 & 36 & 38 & 14 & 35 & 28 & 33 & 0 & 37 & 28 & 12 & 24 & 31 \\
Gen. correct (of 42) & 34 & 39 & 39 & 32 & 36 & 40 & 39 & 0 & 34 & 36 & 23 & 33 & 24 \\
\midrule
\multicolumn{14}{l}{\textbf{Localisation (block lane)}} \\
\midrule
LLI blk med (median) & 0.105 & 0.106 & 0.100 & 0.019 & 0.042 & 0.105 & 0.063 & 0.148 & 0.300 & 0.311 & 0.117 & 0.036 & 0.038 \\
LLI blk gen (median) & 0.128 & 0.105 & 0.144 & 0.036 & 0.048 & 0.144 & 0.088 & 0.146 & 0.139 & 0.275 & 0.119 & 0.035 & 0.041 \\
$N_{eff}$ med & 7.8 & 7.8 & 8.8 & 12.5 & 13.2 & 7.5 & 10.8 & 4.8 & 3.1 & 3.0 & 6.7 & 15.2 & 12.8 \\
$N_{eff}$ gen & 6.7 & 7.8 & 6.4 & 10.4 & 12.2 & 5.8 & 8.6 & 4.8 & 6.0 & 3.4 & 6.6 & 15.3 & 12.4 \\
$N_{eff}/B$ & 0.18 & 0.20 & 0.12 & 0.75 & 0.46 & 0.22 & 0.31 & 0.34 & 0.13 & 0.10 & 0.24 & 0.48 & 0.53 \\
LLI correct & 0.120 & 0.111 & 0.118 & 0.026 & 0.043 & 0.132 & 0.076 & {--} & 0.166 & 0.292 & 0.121 & 0.036 & 0.039 \\
LLI incorrect & 0.103 & 0.076 & 0.107 & 0.020 & 0.045 & 0.100 & 0.054 & 0.147 & 0.316 & 0.299 & 0.114 & 0.034 & 0.039 \\
\midrule
\multicolumn{14}{l}{\textbf{Cross-prompt reuse (block lane)}} \\
\midrule
Jac within (median) & 0.785 & 0.803 & 0.749 & 0.796 & 0.777 & 0.758 & 0.761 & 0.906 & 0.512 & 0.756 & 0.868 & 0.785 & 0.762 \\
Jac across (median) & 0.730 & 0.741 & 0.670 & 0.723 & 0.696 & 0.732 & 0.704 & 0.865 & 0.385 & 0.710 & 0.875 & 0.721 & 0.698 \\
$\Delta$Jac & 0.055 & 0.062 & 0.079 & 0.072 & 0.081 & 0.026 & 0.056 & 0.040 & 0.127 & 0.046 & $-$0.007$^{\mathrm{R}}$ & 0.064 & 0.065 \\
$p$ (Mann-Whitney $U$) & $<$.001 & $<$.001 & $<$.001 & $<$.001 & $<$.001 & $<$.001 & $<$.001 & $<$.001 & $<$.001 & $<$.001 & 0.983$^{\mathrm{R}}$ & $<$.001 & $<$.001 \\
\midrule
\multicolumn{14}{l}{\textbf{Generation floor (block lane)}} \\
\midrule
$N_{com}$ & 10 & 10 & 15 & 3 & 5 & 6 & 7 & 3 & 7 & 5 & 7 & 6 & 4 \\
$N_{flr}$ & 7 & 7 & 7 & 3 & 2 & 5 & 4 & 2 & 2 & 6 & 2 & 2 & 1 \\
$\Delta$LLI & $-$0.044 & $-$0.044 & $-$0.052 & $-$0.009 & $-$0.020 & $-$0.050 & $-$0.031 & $-$0.071 & 0.013 & $-$0.045 & 0.012 & $-$0.016 & $-$0.012 \\
$K_{50}$ & 3.0 & 3.0 & 3.0 & 5.0 & 5.0 & 3.0 & 4.0 & 2.0 & 2.0 & 2.0 & 3.0 & 7.0 & 5.0 \\
$K_{80}$ & 9.0 & 9.0 & 14.0 & 10.0 & 15.0 & 10.0 & 12.5 & 6.0 & 8.0 & 3.0 & 10.0 & 17.0 & 13.0 \\
$N_{com \cap flr}$ & 7 & 6 & 7 & 3 & 2 & 5 & 4 & 2 & 2 & 5 & 2 & 2 & 1 \\
Overlap frac. & 0.700 & 0.545 & 0.467 & 1.000 & 0.400 & 0.833 & 0.571 & 0.667 & 0.286 & 0.833 & 0.286 & 0.333 & 0.250 \\
\midrule
\multicolumn{14}{l}{\textbf{Format compliance (general domain, of 42)}} \\
\midrule
Compliant rate & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 0.881 & 0.190 & 1.000 & 1.000 & 1.000 & 0.810 & 0.976 \\
No answer & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 8 & 0 \\
Verbose & 0 & 0 & 0 & 0 & 0 & 0 & 5 & 34 & 0 & 0 & 0 & 0 & 1 \\
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]
\scriptsize
\setlength{\itemsep}{0pt}\setlength{\parskip}{0pt}\setlength{\topsep}{0pt}
\item Metrics per Eqs.~5, 6, 9, 11, 12; medians over prompts (block lane). $N_{eff}/B$ and $K_{50}/K_{80}$ pool domains.
\item $\dagger$ Mn-3B: correctness-conditioned rows reflect format non-engagement, not knowledge (it rephrases/repeats rather than answering). All other rows are correctness-independent. \{--\}: no correct prompts, so LLI$_{\text{correct}}$ undefined.
\item $^{\mathrm{R}}$ Q-1.7B: $\Delta$Jac reversed and non-significant ($p\geq.05$); all others $\Delta$Jac$>0$, $p<.001$ ($p<.001$ shown as $<$.001).
\item $\Delta$LLI $<0$: removing always-on components lowers apparent localisation. Format compliance (general domain): compliant $=$ non-empty, $\leq$6 words, not repetitive; no answer $=$ empty; verbose $=$ $>$6 words (repetition category omitted, zero for all).
\item Head-lane LLI omitted: near-zero ($\sim$0.0004--0.06) across the cohort.
\end{tablenotes}
\end{threeparttable}
\end{table*}
